FutureMapping: The Computational Structure of Spatial AI Systems

We discuss and predict the evolution of Simultaneous Localisation and Mapping (SLAM) into a general geometric and semantic `Spatial AI' perception capability for intelligent embodied devices. A big gap remains between the visual perception performance that devices such as augmented reality eyewear or comsumer robots will require and what is possible within the constraints imposed by real products. Co-design of algorithms, processors and sensors will be needed. We explore the computational structure of current and future Spatial AI algorithms and consider this within the landscape of ongoing hardware developments.

==> newcom.tex <==
% Content of newcom.tex was merged with symbols.tex.
% 
% You do not need to include this file anymore. This file is here only to ensure 
% backwards compatibility.
 

